TaSL: Continual Dialog State Tracking via Task Skill Localization and Consolidation

A practical dialogue system requires the capacity for ongoing skill acquisition and adaptability to new tasks while preserving prior knowledge. However, current methods for Continual Dialogue State Tracking (DST), a crucial function of dialogue systems, struggle with the catastrophic forgetting issue and knowledge transfer between tasks. We present TaSL, a novel framework for task skill localization and consolidation that enables effective knowledge transfer without relying on memory replay. TaSL uses a novel group-wise technique to pinpoint task-specific and task-shared areas. Additionally, a fine-grained skill consolidation strategy protects task-specific knowledge from being forgotten while updating shared knowledge for bi-directional knowledge transfer. As a result, TaSL strikes a balance between preserving previous knowledge and excelling at new tasks. Comprehensive experiments on various backbones highlight the significant performance improvements of TaSL over existing state-of-the-art methods. The source code is provided for reproducibility.

==> 4.exp_setup.tex <==
%\subsection{Dataset}
\paragraph{Dataset}
We use the continual learning for DST setup proposed by \citet{zhu2022continual}, which uses 15 single domains from the Schema-Guided Dialog dataset (SGD)~\cite{rastogi2020towards}.
We aggregate our results over the same five domain orders to make the most reliable comparisons with prior works.
Comparing results with the same order is crucial as the results
can have significant variance depending on the chosen domains and their order.
More details about data statistics, task selection, and orderings can be found in the Appendix~\ref{sec:dataset}.



\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{l|c|ccc}
\toprule
Method&   Memory-Free & Avg. JGA&  FWT&  BWT \\
\midrule
\rule{0pt}{4pt} Fine-tuning~\cite{madotto2020continual}  &  \multirow{5}*{\tabincell{c}{\cmark}}   & 44.1_{0.9} & 8.3_{1.0} & -36.6_{3.9}  \\
\rule{0pt}{8pt} EWC~\cite{kirkpatrick2017overcoming}  &   & 47.9_{1.1} & 8.4_{0.9} & -38.1_{4.1}  \\
\rule{0pt}{8pt} AdapterCL~\cite{madotto2020continual}   &    & 49.8_{1.7} & - & - \\
\rule{0pt}{8pt} DST-EGQA~\cite{cho2023continual} &    & 55.5_{3.5} & 23.6_{2.1} & -19.1_{4.2}  \\
\rule{0pt}{8pt} \textbf{{\ouralg} (ours)} &   & \textbf{63.1}_{2.0} & \textbf{26.6}_{1.5} & \textbf{-8.1}_{2.2}  \\

\midrule
\rule{0pt}{8pt} Replay~\cite{madotto2020continual}  &  \multirow{3}*{\tabincell{c}{\xmark}}  & 58.6_{3.5} & 10.9_{0.5} & -3.2_{2.3}  \\
\rule{0pt}{8pt} CPT~\cite{zhu2022continual} &    & 61.2_{2.5} & 13.7_{0.8} & 0.5_{0.4} \\
\rule{0pt}{8pt} DST-EGQA~\cite{cho2023continual} &   &  68.9_{0.3} & 22.5_{1.8} & -5.9_{1.9}  \\

\midrule
\rule{0pt}{8pt} CPT Multi-task~\cite{zhu2022continual} & \multirow{2}*{\tabincell{c}{-}}  &  64.0_{1.9} & - & -  \\
\rule{0pt}{8pt} DST-EGQA Multi-task~\cite{cho2023continual} &   & 74.2_{1.8} & - & -  \\

\bottomrule
\end{tabular}}
\caption{CL metric results of different methods at the same T5-small backbone. Means and standard variances are reported. 
%We compare models sequentially trained on 15 tasks from the SGD dataset and aggregate results across five domain permutations. 
The last two rows provide the multi-tasking results, which serve as an upper bound.
Our memory replay-free {\ouralg} outperforms the previous best method, DST-EGQA, by achieving a 7.6\% absolute improvement on avg. JGA and an 11\% increase in BWT. Additionally, it exceeds the performance of the majority of methods that rely on memory replay and nearly matches the upper bound set by the CPT multi-task method.
}
\label{tbl:result}
\end{table*}

%\subsection{Evaluation Protocol}
\paragraph{Evaluation Protocol}
We evaluate DST performance using the widely adopted Joint Goal Accuracy (JGA) metric \cite{wu2019transferable}, which indicates the percentage
of turns for which all slot values are correctly predicted.
We denote $a_{j,i}$ as the JGA on the test set of task $\mathcal{T}_i$ right after training on task $\mathcal{T}_j$.
The performance of Continual DST is assessed using three metrics from \citet{zhu2022continual}: 
\begin{equation}
    \mathbf{Avg.\ JGA} =\frac{1}{K} \sum_{i=1}^{K} a_{K, i}
\end{equation}
\begin{equation}
    \mathbf{FWT} = \frac{1}{K-1} \sum\limits_{i=2}^{K} a_{i-1, i}
\end{equation}
\begin{equation}
    \mathbf{BWT} = \frac{1}{K-1} \sum\limits_{i=1}^{K-1} a_{K, i}-a_{i, i}
\end{equation}
Avg. JGA represents the average JGA across all tasks after training on the final task $\mathcal{T}_K$.
Forward Transfer (FWT) evaluates a model's generalization ability by measuring the averaged zero-shot performance. 
Backward Transfer (BWT) assesses the impact of learning on subsequent tasks on a previous task.
Negative BWT indicates the model lost some previously acquired knowledge.




%\subsection{Baselines and Training Details}
\paragraph{Baselines}
We evaluate our method with the following Continual DST baselines:
\textbf{\emph{Fine-tuning:}} Continuously fine-tune the backbone model on new task data.
\textbf{\emph{Replay:}}
Randomly save $\left| \mathcal{M} \right|$ samples from the training set of each previous task $\mathcal{T}_i$ in memory $\mathcal{M}_i$ and jointly train the model on new task data $\mathcal{D}_K$ and memory $\mathcal{M}_{<k}$.
\textbf{\emph{EWC:}}
Maintain a memory but leverage it to compute the Fisher information matrix for regularization \cite{kirkpatrick2017overcoming}.
\textbf{\emph{AdapterCL:}}
Freeze the pre-trained model and independently train a residual Adapter \cite{houlsby2019parameter} for each task \cite{madotto2020continual}.
\textbf{\emph{Continual Prompt Tuning (CPT) \cite{zhu2022continual}:}}
Freeze the backbone model and continually train soft prompts with memory-guided knowledge transfer in both forward and backward directions.
\textbf{\emph{DST-EGQA \cite{cho2023continual}:}}
Reformulate DST as a QA task to mitigate forgetting with retrieval-augmented in-context learning.



\paragraph{Training Details}
We utilize four distinct parameter-level backbones for experiments: T5-small \cite{raffel2020exploring}, T5-base, Flan-T5-large~\cite{chung2022scaling}, and LLaMA-7B \cite{touvron2023llama}. For the T5 series model, we perform full fine-tuning across all parameters. For LLaMA-7B, we adopt the Parameter-Efficient Fine-Tuning technique, specifically Low-Rank Adaptation (LoRA) \cite{hu2021lora}, to expedite the training process.
In {\ouralg}, the hyperparameters $\alpha_1$ and $\alpha_2$ in Eq. (\ref{eq:I}) and Eq. (\ref{eq:U}) are set to 0.85. Similarly, we set $\beta$ in Eq. \ref{eq:norm} and $\gamma$ in Eq. (\ref{eq:5}) to 0.7.
The memory size per task $\left| \mathcal{M} \right|$ is maintained at 50, aligning with previous studies. Detailed training settings are provided in Appendix \ref{sec:skill_unit}.


